Saliency Can Be All You Need In Contrastive Self-Supervised Learning

We propose an augmentation policy for Contrastive Self-Supervised Learning (SSL) in the form of an already established Salient Image Segmentation technique entitled Global Contrast based Salient Region Detection. This detection technique, which had been devised for unrelated Computer Vision tasks, was empirically observed to play the role of an augmentation facilitator within the SSL protocol. This observation is rooted in our practical attempts to learn, by SSL-fashion, aerial imagery of solar panels, which exhibit challenging boundary patterns. Upon the successful integration of this technique on our problem domain, we formulated a generalized procedure and conducted a comprehensive, systematic performance assessment with various Contrastive SSL algorithms subject to standard augmentation techniques. This evaluation, which was conducted across multiple datasets, indicated that the proposed technique indeed contributes to SSL. We hypothesize whether salient image segmentation may suffice as the only augmentation policy in Contrastive SSL when treating downstream segmentation tasks.

==> Motivation.tex <==
\subsection{Motivation: PVs' Classification}
Learning a classifier for solar panels was a task required by the authors, and became  the main motivation to investigate augmentation policies. 
To this end, the original idea was to obtain a \textit{zero-shot} solar panel segmentation model to crop the panels out of solar arrays, and then map the cropped areas with bounding box annotations -- to formulate a panel/cell classification problem.

\td{ELABORATE on PVs / departure point?}
\vk{I think we shouldn't elaborate more on our departure point as it would distract the reader. Starting from PV array defect classification and then drifting towards this angle might be hard to track.. I suggest we remove this subsection altogether.. Nevertheless, our departure point can even be a standalone paper in which we explain how we started and then converted into cell classification and then used zero shot segmentation as a weak labeling.. quite an applied paper}

==> deleted.tex <==

\begin{figure}[ht]
  \centering
  \includegraphics[width=1.0\columnwidth]{figures/ten_views_simclr.png}
\caption{Ten different views from augmentations (taken from SimCLR~\cite{chen2020simple}).}
\label{figure:ten_augs_simclr}
\end{figure}

The STL-10 is an image dataset derived from ImageNet and popularly used to evaluate algorithms of unsupervised feature learning or self-taught learning.
